Training self-supervised peptide sequence models on artificially chopped proteins

Representation learning for proteins has primarily focused on the global understanding of protein sequences regardless of their length. However, shorter proteins (known as peptides) take on distinct structures and functions compared to their longer counterparts. Unfortunately, there are not as many naturally occurring peptides available to be sequenced and therefore less peptide-specific data to train with. In this paper, we propose a new peptide data augmentation scheme, where we train peptide language models on artificially constructed peptides that are small contiguous subsets of longer, wild-type proteins; we refer to the training peptides as "chopped proteins". We evaluate the representation potential of models trained with chopped proteins versus natural peptides and find that training language models with chopped proteins results in more generalized embeddings for short protein sequences. These peptide-specific models also retain information about the original protein they were derived from better than language models trained on full-length proteins. We compare masked language model training objectives to three novel peptide-specific training objectives: next-peptide prediction, contrastive peptide selection and evolution-weighted MLM. We demonstrate improved zero-shot learning performance for a deep mutational scan peptides benchmark.

==> sections/relatedwork.tex <==
%Proteins play a critical role in various biological processes. Protein sequence is a linear ordering of amino acid residues and can be considered as the language of life. 
%
%Given, a n-length protein made from 20 amino acid residues there are $20^n$ possible sequences and sequence is known to encode evolutionary information, structural properties and function.
% \hr{Check if this sounds better}
%
%Protein sequence is the language of life, where amino acids residues are the vocabulary, forming diverse %sentences of protein sequences, with distinctive dialects for the same proteins across species.
%
%
%
Various researchers have noticed the similarity between sequence data from natural languages and protein primary sequences, developing language-inspired protein sequence models~\cite{esm, prottrans, heinzinger2019modeling, alley2019unified, bepler2019learning, he2021pre, madani2020progen, detlefsen2022learning, rao2020transformer}.
These models use self-supervised techniques, such as masked language modeling (MLM) as proposed in BERT~\cite{devlin2018bert},
to learn from the large volume of individual natural protein sequences obtained primarily through next generation genome sequencing. 
%
Protein sequence models are used for downstream tasks such as mutational effect evaluation~\cite{riesselman2018deep, esm, hsu2021combining, meier2021language}
protein function prediction~\cite{gligorijevic2021structure, wang2021lm, stephan2021bridging}
% [refs: DeepFRI, LM-GVP]
, protein-ligand binding \cite{kalakoti2022transdti}, protein-protein interactions~\cite{cheng2021bertmhc}
% [refs: BERTMHC, ]
, protein design \cite{madani2020progen}, and even inferring evolutionary directions~\cite{detlefsen2022learning, hie2022evolutionary}. 
%Vig et al.~\cite{vig2020bertology} found that attention in protein models captures the amino acid contacts in 3D folded protein structures as well as functional binding sites.
%Although we follow many other authors in utilizing a Transformer-based approach~\cite{vaswani2017attention}, a recent study by Yang et al.~\cite{yang2022convolutions} suggests a convolution-based architecture such as dilated CNN achieved competitive performance.

Other objectives have also been adopted in training protein sequence models. For instance, McDermott et al.~\cite{mcdermott2021adversarial} 
introduced adversarial MLM, where an adversarial token masking model is trained jointly with the MLM objective. Inspired from Contrastive Predictive Coding (CPC)~\cite{van2018representation}, the
CPCProt model~\cite{lu2020self}
was developed to use InfoNCE contrastive loss to maximize the mutual information between protein context and local embedding space.
%
He et al.~\cite{he2021pre} use pairwise MLM (PMLM) to explicitly consider dependencies among masked amino acids.
Others explicitly incorporate a proteins’ 3D structural information, from amino acid residue contact maps~\cite{bepler2019learning} or from tertiary structure~\cite{mansoor2021toward}.

% Protein sequence models can also be trained from sets of protein sequences, using multiple sequence alignments (MSAs) that combine multiple evolutionarily-related protein sequences to form a matrix of amino acids. MSA Transformer~\cite{rao2021msa}
% is a transformer-based protein sequence models explicitly learning the evolutionary relatedness from MSA. Prominent deep learning systems including RoseTTAFold~\cite{baek2021accurate} and AlphaFold2~\cite{jumper2021highly} also depend on MSAs to predict protein's 3D structure from its sequence. 
% Unfortunately, in comparison to wild-type (WT) protein sequences, high-quality MSAs are not available for most peptides.

Recent works~\cite{cheng2021pepformer, serrano2020deepmspeptide} have also focused explicitly on peptide sequences, training transformer and convolution-based models to predict peptide detectability by mass spectrometry. However, these approaches involve supervised training over mass spec data, and do not explore leveraging 
large-scale proteomic data with self-supervised learning.


==> sections/resultfiles/TablePeptideContexts.tex <==
\ExplSyntaxOn
\NewDocumentCommand { \getmaxpep } { }
  {
    \clist_gset:Nx \g_tmpa_clist {\baseline, \bmlm, \contrs, \mlm, \nsp}
    \clist_sort:Nn \g_tmpa_clist
      {
        \fp_compare:nNnTF {##1} < {##2}
          { \sort_return_swapped: }
          { \sort_return_same: }
      }
    \tl_gset:Nx \g_tmpa_tl { \clist_item:Nn \g_tmpa_clist {1} }
  }
\NewDocumentCommand { \mynum } { m }
  {
    \fp_compare:nNnTF { #1 } = { \g_tmpa_tl }
      { \cellcolor{blue!20} \num{#1} }
      { \num{#1} }
  }
\ExplSyntaxOff


\def\mywidth{1.7cm}
%\newgeometry{left=1cm,bottom=0.1cm}
\noindent\begin{table*}%[h]
  \sisetup{round-mode=places, round-precision=4}
  \centering
  \caption{\textbf{Accuracies for predicting masked peptide contexts, with the number of masked neighbors (on both sides) indicated in the first column.} }
  \csvreader[tabular=lP{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth},
            table head=\toprule \thead{ Context length \\masked} & \thead{ESM-1b} & \thead{Pept.\\BMLM} & \thead{Pept.\\CNSP} & \thead{Pept.\\MLM} & \thead{Pept.\\MLM-NSP} \\ \midrule,
            head to column names,
            before line=\getmaxpep,
            %late after line = \\\hline,
            late after last line=\\\bottomrule]
            {sections/resultfiles/peptidecontexteval.csv}%
            {}%
            {\csvcoli & \mynum{\baseline} & \mynum{\bmlm} & \mynum{\contrs}  &%
             \mynum{\mlm} & \mynum{\nsp}
            }

  \label{tab:peptidecontextacc}
\end{table*}
%\restoregeometry


==> sections/resultfiles/TableTAPEss3peptides.tex <==
\ExplSyntaxOn
\NewDocumentCommand { \getmax } { }
  {
    \clist_gset:Nx \g_tmpa_clist {\A, \B, \C, \D, \E, \F, \G, \H}
    \clist_sort:Nn \g_tmpa_clist
      {
        \fp_compare:nNnTF {##1} < {##2}
          { \sort_return_swapped: }
          { \sort_return_same: }
      }
    \tl_gset:Nx \g_tmpa_tl { \clist_item:Nn \g_tmpa_clist {1} }
  }
\NewDocumentCommand { \mynum } { m }
  {
    \fp_compare:nNnTF { #1 } = { \g_tmpa_tl }
      { \cellcolor{blue!20} \num{#1} }
      { \num{#1} }
  }
\ExplSyntaxOff


\def\mywidth{1.7cm}
%\newgeometry{left=1cm,bottom=0.1cm}
\noindent\begin{table*}%[h]
  \sisetup{round-mode=places, round-precision=4}
  \centering
  \caption{\textbf{TAPE secondary structure evaluation on peptides in the test sets.} Average accuracy over 3 iterations x 3 random seeds is shown, for each model. 'Winning' model for each test set is highlighted in blue. }
  
  \csvreader[tabular=lP{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth},
            table head=\toprule \thead{ Test set \\(\# peptides)} & \thead{ESM-1b} & \thead{Pept.\\Blosim} & \thead{Pept.\\BMLM} & \thead{Pept.\\CNSP} & \thead{Pept. (70e)\\Contras.} & \thead{Pept.\\MLM} & \thead{Pept.\\MLM-NSP} & \thead{Pept. (70e)\\MLM-NSP} \\ \midrule,
            head to column names,
            before line=\getmax,
            %late after line = \\\hline,
            late after last line=\\\bottomrule]
            {sections/resultfiles/TAPEss3peptides.csv}%
            {}%
            {\csvcoli & \mynum{\A} & \mynum{\B} & \mynum{\C}  &%
             \mynum{\D} & \mynum{\E} & \mynum{\F} & \mynum{\G} & \mynum{\H}
            }
  
  \label{tab:tapess3peptides}
\end{table*}
%\restoregeometry


==> sections/resultfiles/TableTAPEss3proteins.tex <==
\ExplSyntaxOn
\NewDocumentCommand { \getmax } { }
  {
    \clist_gset:Nx \g_tmpa_clist {\A, \B, \C, \D, \E, \F, \G, \H}
    \clist_sort:Nn \g_tmpa_clist
      {
        \fp_compare:nNnTF {##1} < {##2}
          { \sort_return_swapped: }
          { \sort_return_same: }
      }
    \tl_gset:Nx \g_tmpa_tl { \clist_item:Nn \g_tmpa_clist {1} }
  }
\NewDocumentCommand { \mynum } { m }
  {
    \fp_compare:nNnTF { #1 } = { \g_tmpa_tl }
      { \cellcolor{blue!20} \num{#1} }
      { \num{#1} }
  }
\ExplSyntaxOff


\def\mywidth{1.7cm}
%\newgeometry{left=1cm,bottom=0.1cm}
\noindent\begin{table*}%[h]
  \sisetup{round-mode=places, round-precision=4}
  \centering
  \caption{\textbf{TAPE secondary structure evaluation on proteins in the test sets.} Average accuracy over 3 iterations x 3 random seeds is shown, for each model. 'Winning' model for each test set is highlighted in blue. }
  
  \csvreader[tabular=lP{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth},
            table head=\toprule \thead{ Test set \\(\# proteins)} & \thead{ESM-1b} & \thead{Pept.\\Blosim} & \thead{Pept.\\BMLM} & \thead{Pept.\\CNSP} & \thead{Pept. (70e)\\Contras.} & \thead{Pept.\\MLM} & \thead{Pept.\\MLM-NSP} & \thead{Pept. (70e)\\MLM-NSP} \\ \midrule,
            head to column names,
            before line=\getmax,
            %late after line = \\\hline,
            late after last line=\\\bottomrule]
            {sections/resultfiles/TAPEss3proteins.csv}%
            {}%
            {\csvcoli & \mynum{\A} & \mynum{\B} & \mynum{\C}  &%
             \mynum{\D} & \mynum{\E} & \mynum{\F} & \mynum{\G} & \mynum{\H}
            }
  
  \label{tab:tapess3proteins}
\end{table*}
%\restoregeometry


==> sections/resultfiles/TableTAPEstability.tex <==
\ExplSyntaxOn
\NewDocumentCommand { \getmaxstab } { }
  {
    \clist_gset:Nx \g_tmpa_clist {\baseline, \blosim, \bmlm, \contrs, \contrslong, \mlm, \nsp, \nsplong}
    \clist_sort:Nn \g_tmpa_clist
      {
        \fp_compare:nNnTF {##1} < {##2}
          { \sort_return_swapped: }
          { \sort_return_same: }
      }
    \tl_gset:Nx \g_tmpa_tl { \clist_item:Nn \g_tmpa_clist {1} }
  }
% \NewDocumentCommand { \mynum } { m }
%   {
%     \fp_compare:nNnTF { #1 } = { \g_tmpa_tl }
%       { \cellcolor{blue!20} \num{#1} }
%       { \num{#1} }
%   }
\ExplSyntaxOff


\def\mywidth{1.7cm}
%\newgeometry{left=1cm,bottom=0.1cm}
\noindent
%\begin{table*}%[h]
%  \sisetup{round-mode=places, round-precision=4}
%  \centering
%  \caption{\textbf{TAPE stability evaluation in the test sets.} Average Spearman's $\rho$ over 3 random seeds is shown, for each model. The bottom row shows the standard deviations for each model across all iterations. 'Winning' model for each test set is highlighted in blue. }
%  
%  \csvreader[tabular=lP{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth}P{\mywidth},
%            table head=\toprule \thead{ Test set \\(\# proteins)} & \thead{ESM-1b} & \thead{Pept.\\BloSim} & \thead{Pept.\\BMLM} & \thead{Pept.\\C-NPP} & \thead{Pept.\\MLM} & \thead{Pept.\\NPP}\\ \midrule,
%            head to column names,
%            before line=\getmaxstab,
%            %late after line = \\\hline,
%            late after last line=\\\bottomrule]
%            {sections/resultfiles/TAPEstability.csv}%
%            {}%
%            {\csvcoli & \mynum{\baseline} & \mynum{\blosim} & \mynum{\bmlm} & \mynum{\contrs} &%
%             \mynum{\mlm} & \mynum{\nsp} 
%            }
%  
%  \label{tab:tapestability}
%\end{table*}
%\restoregeometry

